Cross-Platform Performance Portability Using Highly Parametrized SYCL Kernels

Over recent years heterogeneous systems have become more prevalent across HPC systems, with over 100 supercomputers in the TOP500 incorporating GPUs or other accelerators. These hardware platforms have different performance characteristics and optimization requirements. In order to make the most of multiple accelerators a developer has to provide implementations of their algorithms tuned for each device. Hardware vendors provide libraries targeting their devices specifically, which provide good performance but frequently have different API designs, hampering portability. The SYCL programming model allows users to write heterogeneous programs using completely standard C++, and so developers have access to the power of C++ templates when developing compute kernels. In this paper we show that by writing highly parameterized kernels for matrix multiplies and convolutions we achieve performance competitive with vendor implementations across different architectures. Furthermore, tuning for new devices amounts to choosing the combinations of kernel parameters that perform best on the hardware.

==> Makefile <==

# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = sc2019.tex

PICS = \
			 pictures/arm_vgg.png \
			 pictures/arm_resnet.png \
			 pictures/intel_vgg.png \
			 pictures/intel_resnet.png \
			 pictures/register_usage.png \
			 pictures/register_spill.png \
			 pictures/amd_register_usage.png \
			 pictures/amd_number_wavefronts.png \
			 pictures/amd_tiled_perf.png \
			 pictures/chromebook_tiled_perf.png \
			 pictures/Matmul-register.png \
			 pictures/Matmul.png \
			 pictures/Matmul-local.png \
			 pictures/Matmul-register-2.png \
			 pictures/gemm_group_4x4_8x8_arm.png \
			 pictures/gemm_group_8x4_4x8_arm.png \
			 pictures/gemm_group_8x4_8x16_arm.png \
			 pictures/gemm_comp_arm.png \
			 pictures/gemm_intel_pre-fetched_nonlog.png \
			 pictures/gemm_intel_pre-fetched.png \
			 pictures/gemm_intel_square_register.png \
			 pictures/gemm_comp_intel.png

TABLES = \
				 data/vgg_layers.csv \
				 data/resnet_layers.csv

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF} ${PICS}

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst %.bib ${PICS} ${TABLES}
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	  do pdflatex $<; done

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

package: ${PICS} ${SAMPLES} ${PDF}
	zip sc2019.zip ${PICS} sc2019.tex sc2019.bbl ${PACKAGE}.cls ${TABLES} ACM-Reference-Format.bst sc2019.bib Makefile

pictures/arm_vgg.png: data/arm_vgg.csv ./scripts/plot_dnn_perf_comparisons.py
	python3 scripts/plot_dnn_perf_comparisons.py data/arm_vgg.csv pictures/arm_vgg.png

pictures/arm_resnet.png: data/arm_resnet.csv ./scripts/plot_dnn_perf_comparisons.py
	python3 scripts/plot_dnn_perf_comparisons.py data/arm_resnet.csv pictures/arm_resnet.png --fullpage

pictures/intel_vgg.png: data/intel_vgg.csv ./scripts/plot_dnn_perf_comparisons.py
	python3 scripts/plot_dnn_perf_comparisons.py data/intel_vgg.csv pictures/intel_vgg.png --batch=4

pictures/intel_resnet.png: data/intel_resnet.csv ./scripts/plot_dnn_perf_comparisons.py
	python3 scripts/plot_dnn_perf_comparisons.py data/intel_resnet.csv pictures/intel_resnet.png --fullpage --batch=4

pictures/amd_register_usage.png: data/amd_gpu.occupancy scripts/register_usage.py
	python3 scripts/register_usage.py data/amd_gpu.occupancy pictures/amd_register_usage.png pictures/amd_number_wavefronts.png --codexl

pictures/register_usage.png: data/register_usage.csv scripts/register_usage.py
	python3 scripts/register_usage.py data/register_usage.csv pictures/register_usage.png pictures/register_spill.png

pictures/chromebook_tiled_perf.png: data/chromebook_tiled_3x3.csv scripts/plot_tile_perf.py
	python3 scripts/plot_tile_perf.py data/chromebook_tiled_3x3.csv pictures/chromebook_tiled_perf.png --use_fast_div

pictures/amd_tiled_perf.png: data/amd_tiled_perf.csv scripts/plot_tile_perf.py
	python3 scripts/plot_tile_perf.py data/amd_tiled_perf.csv pictures/amd_tiled_perf.png

pictures/gemm_group_4x4_8x8_arm.png: scripts/roofline/analyze.py \
                                     scripts/roofline/draw.py \
                                     scripts/roofline/data.py \
                                     data/arm_8_4_8_16_noloc.json \
                                     data/arm_8_4_4_8_noloc.json \
                                     data/arm_4_4_8_8_noloc.json \
                                     data/arm_acl.json
	python3 ./scripts/roofline/analyze.py \
		-g 8_4_8_16_noloc data/arm_8_4_8_16_noloc.json \
		-g 8_4_4_8_noloc data/arm_8_4_4_8_noloc.json \
		-g 4_4_8_8_noloc data/arm_4_4_8_8_noloc.json \
		-g "ACL CL Gemm" data/arm_acl.json \
		-x 12.5 32 -y 7 46 -t avg_event_time -p 2 -s 30 60 -a 2.8 --no-legend -d 2 0 \
		-o pictures/gemm_group_4x4_8x8_arm.png

pictures/gemm_group_8x4_4x8_arm.png: scripts/roofline/analyze.py \
                                     scripts/roofline/draw.py \
                                     scripts/roofline/data.py \
                                     data/arm_8_4_8_16_noloc.json \
                                     data/arm_8_4_4_8_noloc.json \
                                     data/arm_4_4_8_8_noloc.json \
                                     data/arm_acl.json
	python3 ./scripts/roofline/analyze.py \
	 -g 8_4_8_16_noloc data/arm_8_4_8_16_noloc.json \
	 -g 8_4_4_8_noloc data/arm_8_4_4_8_noloc.json \
	 -g 4_4_8_8_noloc data/arm_4_4_8_8_noloc.json \
	 -g "ACL CL Gemm" data/arm_acl.json -x 28 47 -y 30 150 -t avg_event_time \
	 -p 5 -s 30 60 -a 2.7 --no-legend -d 2 0 \
	 -o pictures/gemm_group_8x4_4x8_arm.png

pictures/gemm_group_8x4_8x16_arm.png: scripts/roofline/analyze.py \
                                      scripts/roofline/draw.py \
                                      scripts/roofline/data.py \
                                      data/arm_8_4_8_16_noloc.json \
                                      data/arm_8_4_4_8_noloc.json \
                                      data/arm_4_4_8_8_noloc.json \
                                      data/arm_acl.json
	python3 ./scripts/roofline/analyze.py \
	 -g 8_4_8_16_noloc data/arm_8_4_8_16_noloc.json \
	 -g 8_4_4_8_noloc data/arm_8_4_4_8_noloc.json \
	 -g 4_4_8_8_noloc data/arm_4_4_8_8_noloc.json \
	 -g "ACL CL Gemm" data/arm_acl.json -x 67 158 -y 82 135 -t avg_event_time \
	 -s 30 60 -a 2.8 --no-legend -d 2 0 \
	 -o pictures/gemm_group_8x4_8x16_arm.png

pictures/gemm_comp_arm.png: scripts/roofline/analyze.py \
                            scripts/roofline/draw.py \
                            scripts/roofline/data.py \
                            data/arm_8_4_8_16_noloc.json \
                            data/arm_8_4_4_8_noloc.json \
                            data/arm_4_4_8_8_noloc.json \
                            data/arm_acl.json
	python3 ./scripts/roofline/analyze.py \
	 -g 8x4_8x16_noloc data/arm_8_4_8_16_noloc.json \
	 -g 8x4_4x8_noloc data/arm_8_4_4_8_noloc.json \
	 -g 4x4_8x8_noloc data/arm_4_4_8_8_noloc.json \
	 -g "ACL CL Gemm" data/arm_acl.json -x 10 210 -y 2.9 170 -t avg_event_time \
	 --draw-boxes -d 2 0 -a 1.5 \
	 -o pictures/gemm_comp_arm.png

pictures/gemm_intel_pre-fetched_nonlog.png: scripts/roofline/analyze.py \
                                            scripts/roofline/draw.py \
                                            scripts/roofline/data.py \
                                            data/intel_8_4_8_16_loc.json \
                                            data/intel_8_4_8_16_ndb.json
	python3 ./scripts/roofline/analyze.py \
	 -g "With double buffering" data/intel_8_4_8_16_loc.json \
	 -g "Without double buffering" data/intel_8_4_8_16_ndb.json -x 10 150 -t avg_event_time \
	 -y 0 280 --ynolog -d 3 1 \
	 -o pictures/gemm_intel_pre-fetched_nonlog.png

pictures/gemm_intel_pre-fetched.png: scripts/roofline/analyze.py \
                                     scripts/roofline/draw.py \
                                     scripts/roofline/data.py \
                                     data/intel_8_4_8_16_loc.json \
                                     data/intel_8_4_8_16_ndb.json
	python3 ./scripts/roofline/analyze.py \
	 -g "With double buffering" data/intel_8_4_8_16_loc.json \
	 -g "Without double buffering" data/intel_8_4_8_16_ndb.json -x 13 145 -t avg_event_time \
	 -y 50 300 -d 3 1 -s 30 60 \
	 -o pictures/gemm_intel_pre-fetched.png

pictures/gemm_intel_square_register.png: scripts/roofline/analyze.py \
	                                       scripts/roofline/draw.py \
	                                       scripts/roofline/data.py \
	                                       data/intel_4_4_8_8_loc.json \
	                                       data/intel_8_2_4_16_loc.json
	python3 ./scripts/roofline/analyze.py \
	 -g "Square tile (4x4_8x8)" data/intel_4_4_8_8_loc.json \
	 -g "Non-square tile (8x2_4x16)" data/intel_8_2_4_16_loc.json -x 10 150 -t avg_event_time \
	 -y 55 240 -d 3 1 -s 30 60 \
	 -o pictures/gemm_intel_square_register.png

pictures/gemm_comp_intel.png: scripts/roofline/analyze.py \
                              scripts/roofline/draw.py \
                              scripts/roofline/data.py \
                              data/intel_4_4_8_8_loc.json \
                              data/intel_8_4_8_16_loc.json \
                              data/intel_4_4_16_16_loc.json \
                              data/intel_clblast.json
	python3 ./scripts/roofline/analyze.py \
	 -g 4x4_8x8_loc data/intel_4_4_8_8_loc.json \
	 -g 8x4_8x16_loc data/intel_8_4_8_16_loc.json \
	 -g 4x4_16x16_loc data/intel_4_4_16_16_loc.json \
	 -g clblast data/intel_clblast.json -x 12.5 140 -t avg_event_time \
	 -y 35 320 -d 3 1 \
	 -o pictures/gemm_comp_intel.png

clean_pictures:
	$(RM) ${PICS}

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ samples/sample-*.pdf *.cls *.bst

